Efficient Online Bandit Multiclass Learning with $\tilde{O}(\sqrt{T})$ Regret

We present an efficient second-order algorithm with $\tilde{O}(\frac{1}{\eta}\sqrt{T})$ regret for the bandit online multiclass problem. The regret bound holds simultaneously with respect to a family of loss functions parameterized by $\eta$, for a range of $\eta$ restricted by the norm of the competitor. The family of loss functions ranges from hinge loss ($\eta=0$) to squared hinge loss ($\eta=1$). This provides a solution to the open problem of (J. Abernethy and A. Rakhlin. An efficient bandit algorithm for $\sqrt{T}$-regret in online multiclass prediction? In COLT, 2009). We test our algorithm experimentally, showing that it also performs favorably against earlier algorithms.

==> basic_algorithm.tex <==
\section{A Basic Algorithm}
\begin{algorithm}
\caption{Basic Second Order Banditron Algorithm (Basic-SOBA)}
\label{alg:basic-soba}
\begin{algorithmic}
\REQUIRE Regularization parameter $a \geq 0$, exploration parameter $\gamma \in [0,1]$.
\STATE Initialization: $\bm W_1 = 0 \in \R^{k \times d}$
\FOR{$t = 1,2,\ldots,m$}
\STATE Receive $\bm x_t \in \R^d$
\STATE Compute $\hat{y}_t = \arg\max_{i \in [k]} (\bm W_t \bm x_t)_i$
\STATE %Define $p_{t,i} = (1-\gamma)\one[i=\hat{y}_t]+\tfrac{\gamma}{k}$ for $i \in [k]$
       Define $\bm p_t = (1 - \gamma)e_{\hat{y}_t} + \frac{\gamma}{k} \one_k$
\STATE Randomly sample $\tilde{y}_t$ according to $\bm p_t$
\STATE Receive feedback $\one[\tilde{y}_t = y_t]$
\IF{$\hat{y}_t \neq \tilde{y}_t = y_t$}
\STATE Compute loss gradient $\bm g_t = \frac{\one[\tilde{y}_t = y_t]}{p_{t,y_t}} (\bm e_{\hat{y}_t} - \bm e_{y_t}) \otimes \bm x_t$
\STATE Compute adaptive regularization term $\bm z_t = \sqrt{p_{t,y_t}} \bm g_t$
\ELSE
\STATE $z_t = 0$, $g_t = 0$
\ENDIF
\STATE Compute adaptive regularizer $\bm A_t = a \bm I + \sum_{s=1}^t \bm z_s \bm z_s^T$
\STATE Update $\bm W_{t+1} \gets \bm A_{t}^{-1} (-\sum_{s=1}^{t} \bm g_s)$
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> result_chicheng.tex <==
\section{Main Result}
\label{sec:main_result}

\begin{algorithm}
\caption{Second Order Banditron Algorithm}
\label{alg:sop-banditron}
\begin{algorithmic}[1]
\STATE Initialization: $W_1 = 0 \in \R^{k \times d}$
\FOR{$t = 1,2,\ldots,m$}
\STATE Set $\hat{y}_t = \arg\max_{k} ({W_t}^T x_t)_k$
\STATE Set $p_{t,i} = (1-\gamma)I[i=\hat{y}_t]+\tfrac{\gamma}{k}$ for $i \in [k]$
\STATE Randomly sample $\tilde{y}_t$ according to $p_t$
\STATE Receive feedback $I[\tilde{y}_t = y_t]$
\STATE Set $g_t = \frac{I[y_t = \tilde{y}_t]}{p_{t,y_t}} x_t \otimes (e_{\hat{y}_t} - e_{y_t})$
\STATE Set $z_t = \sqrt{p_{t,y_t}} g_t$
\STATE Set $A_t = a I + \sum_{s=1}^t z_s z_s^T$
\STATE $W_{t+1} \gets A_{t}^{-1} (-\sum_{s=1}^{t} g_s)$
\ENDFOR
\end{algorithmic}
\end{algorithm}

%: a $O(\sqrt{T})$-regret Algorithm
Our plan in this section is to develop a regret bound based on a specific time-varying elliptic
potential. We analyze the $\gamma$-greedy algorithm, and as a first step we bound
the performance of $\hat{y}_t$. Throughout,
suppose all the examples are $\ell_2$-bounded, i.e. $\|x_t\| \leq X$.

Define a new estimator of the gradient as
\[
g_t = \frac{I[y_t = \tilde{y}_t]}{p_{t,y_t}} x_t \otimes (e_{\hat{y}_t} - e_{y_t}),
\]
We associate a time-varying regularizer $R_t(w) = \frac12\| w \|_{A_{t-1}}^2$,
where $A_t = a I + \sum_{s=1}^t z_s z_s^T$ and
\[
z_t = \sqrt{p_{t,y_t}} g_t = \frac{I[y_t = \tilde{y}_t]}{\sqrt{p_{t,y_t}}} x_t \otimes (e_{\hat{y}_t} - e_{y_t})~.
\]
Note that the estimator $g_t$ has the nice property that it is nonzero only if
$y_t = \tilde{y}_t \neq \hat{y}_t$. That is, it only makes an update when the
algorithm is exploring and the exploration label $\tilde{y}_t$ ``luckily'' hits
the true label $y_t$.


In this case, $p_{t,y_t} = \frac{\gamma}{k}$
holds determinstically. Therefore, we can rewrite $g_t$ and $z_t$ as
\begin{align*}
g_t &= \frac{k I[y_t = \tilde{y}_t \neq \hat{y}_t]}{\gamma} x_t \otimes (e_{y_t} - e_{\hat{y}_t}),\\
z_t &= \sqrt{\frac{\gamma}{k}} g_t
    = \sqrt{\frac{k I[y_t = \tilde{y}_t \neq \hat{y}_t]}{\gamma}} x_t \otimes (e_{y_t} - e_{\hat{y}_t})~.
\end{align*}

We also have
\begin{align}
\E_{t-1} [g_t] &= x_t \otimes (e_{\hat{y}_t} - e_{y_t}) \label{eq:expectation_g} \\
\E_{t-1} [\inn{W}{z_t}^2] &= \inn{W}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})}^2~. \label{eq:expectation_z2}
\end{align}
%By standard results on FTRL using time varying regularizers(See,
%for example, Lemma 1 of~\cite{Orabona-Crammer-Cesa-Bianchi-2015})
%, if $W_t = \nabla R_t(-\sum_{s=1}^{t-1} g_s)$, we have
%\[ \sum_{t=1}^T \inn{W_t - W^*}{g_t} \leq \frac12 \| W^* \|_{A_T}^2 + \frac12\sum_{t=1}^T \| g_t \|_{A_{t-1}^{-1}}^2 \]
%Taking expectations on both sides,
%\begin{eqnarray}
%\E[\sum_{t=1}^T \inn{W_t - W^*}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})}]
%&\leq&
%\frac12 \E[a \| W^* \|^2 + \sum_{t=1}^T (\inn{W^*}{z_t})^2 + \sum_{t=1}^T \tr(A_{t-1}^{-1} (g_t g_t^T))] \nonumber \\
%&=&
%\frac12 \E[a \| W^* \|^2 + \sum_{t=1}^T (\inn{W^*}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})})^2 + \sum_{t=1}^T \tr(A_{t-1}^{-1} (g_t g_t^T))]
%\label{eqn:notquitevaw}
%\end{eqnarray}

%Note that we cannot use a Vovk-Azoury-Warmuth like forecaster,
%since at round $t$, we are not able to observe $z_t$ (specifically $y_t$
%is unseen). Would it have been the case, we will end up bounding
%$\sum_{t=1}^T \tr(A_t^{-1} (g_t g_t^T))$, which is automatically $\frac{d\ln T}{p_{\min}}$.
%Here, instead we establish a technical lemma, carefully bounding the last term.

%\begin{lemma}
%Let $p_{\min}:=\min\{p_{t,y_t}: g_t \neq 0\}$. Then,
%\[ \sum_{t=1}^T \tr(A_{t-1}^{-1} (g_t g_t^T)) \leq (\frac{1}{p_{\min}})^2 \frac{dX^2}{a} + \frac{1}{p_{\min}} d \ln(1 + \frac{TX^2}{a p_{\min}d}) \]
%\end{lemma}
%\paragraph{Remark.} Note if $\gamma$-greedy strategy is deployed, $p_{\min} \geq \frac{k}{\gamma}$. Therefore, the above can further bounded as
%\[ (\frac{k}{\gamma})^2 \frac{dX^2}{a} + \frac{k}{\gamma} d \ln(1 + \frac{TX^2 k}{a d \gamma}) \]
%The bound in the last term can be slightly refined: we can replace $T$ with
%$\sum_{t=1}^T I(\tilde{y}_t = y_t \neq \hat{y}_t)$.

%\begin{proof}
%\begin{eqnarray*}
%&& \sum_{t=1}^T \tr(A_{t-1}^{-1} (g_t g_t^T)) \\
%&=& \sum_{t=1}^T \tr((A_{t-1}^{-1} - A_t^{-1}) (g_t g_t^T)) + \tr(A_t^{-1} (g_t g_t^T)) \\
%&\leq& \sum_{t=1}^T \tr(A_{t-1}^{-1} - A_t^{-1}) \cdot \| g_t g_t^T \|_2 + \tr(A_t^{-1} (z_t z_t^T)) \frac{1}{p_{t,y_t}} \\
%&\leq& (\max_t  \| g_t g_t^T \|_2) \sum_{t=1}^T \tr(A_{t-1}^{-1} - A_t^{-1})
%+ (\max_t \frac{1}{p_{t,y_t}}) \sum_{t=1}^T \ln \frac{\det(A_t)}{\det(A_{t-1})} \\
%&\leq& \frac{X^2}{p_{\min}^2} \tr(A_0^{-1}) + \frac{1}{p_{\min}} \ln \det(A_0^{-1} A_T) \\
%&\leq& (\frac{1}{p_{\min}})^2 \frac{dX^2}{a} + \frac{1}{p_{\min}} d \ln(1 + \frac{TX^2}{a p_{\min}d})
%\end{eqnarray*}
%\end{proof}

%Continuing Equation~\eqref{eqn:notquitevaw}, we have
%\[
%\E[\sum_{t=1}^T \inn{W_t - W^*}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})}]
%\leq
%\frac12 \E[a \| W^* \|^2 + \sum_{t=1}^T (\inn{W^*}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})})^2 + (\frac{k}{\gamma})^2 \frac{dX^2}{a} + \frac{k}{\gamma} d \ln(1 + \frac{TX^2 k}{a d \gamma}) ]
%\]
%Now, notice that $z_t \neq 0$ only if $y_t \neq \hat{y}_t$, the above can be
%rewritten as
%\[
%\E[\sum_{t=1}^T \inn{W_t - W^*}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})} I(y_t \neq \hat{y_t}) ]
%\leq
%\frac12 \E[a \| W^* \|^2 + \sum_{t=1}^T (\inn{W^*}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})})^2I(y_t \neq \hat{y_t}) + (\frac{k}{\gamma})^2 \frac{dX^2}{a} + \frac{k}{\gamma} d \ln(1 + \frac{TX^2 k}{a d \gamma}) ]
%\]

%Adding $\sum_{t=1}^T b I(\hat{y}_t \neq y_t)$ on both sides and noticing that $\inn{W_t}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})} \geq 0$
%, we obtain
%\begin{eqnarray}
%&&\E[\sum_{t=1}^T I(\hat{y}_t \neq y_t) b] \nonumber \\
%&\leq&\E[\sum_{t=1}^T I(\hat{y}_t \neq y_t) (b - \inn{W_t}{x_t \otimes (e_{y_t} - e_{\hat{y}_t})})] \nonumber \\
%&\leq&
%\E[\sum_{t=1}^T I(\hat{y}_t \neq y_t)
%(b - \inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t})}
%+
%\frac{1}{2}\inn{W^*}{x_t \otimes (e_{\hat{y}_t} - e_{y_t})}^2)
%+
%\frac{a}{2} \| W^* \|^2
%+
%(\frac{k}{\gamma})^2 \frac{dX^2}{a} + \frac{k}{\gamma} d \ln(1 + \frac{TX^2 k}{a d \gamma}) ]
%\nonumber \\
%\label{eqn:mbgeneral}
%\end{eqnarray}

%\subsection{Fixing the +1 Issue}
%\subsubsection{A Crucial Lemma}
%In this subsection, w
We first show the following lemma. Note that this is a statement over any sequence and no expectation is taken.
%
\begin{lemma}
\label{lem:vaw}
For any $U \in \R^{k \times d}$, we have:
\begin{align*}
&\sum_{t=1}^T \left(2 \inn{U}{-g_t} - \inn{U}{z_t}^2 \right)\\
&\quad \leq a  \| U\|^2 + \frac {k^2} {\gamma} d \ln\left(1 + \frac{2TX^2k}{a \gamma d}\right)~.
\end{align*}
\end{lemma}
%
\begin{proof}
%Following~\cite{Orabona-Cesa-Bianchi-Gentile-2012},
We reduce to proof to the regret analysis of online least squares problem.
Define $u = \sqrt{\frac{k}{\gamma}}$.
Recall that
$z_t = \frac1u g_t = \sqrt{\frac \gamma k} g_t =
\sqrt{\frac{k\,I[y_t = \tilde{y}_t \neq \hat{y}_t]}{\gamma}} x_t \otimes (e_{\hat{y}_t} - e_{y_t})$,
%and
%$u_t = \sqrt{\frac{k}{\gamma}}$.
and $A_t = aI + \sum_{s=1}^t z_s z_s^T$, and
$W_t$ is the ridge regression solution based on data collected in time $1$ to $t-1$,
i.e. $W_t = A_{t-1}^{-1} (-\sum_{s=1}^{t-1} g_s) = A_{t-1}^{-1} (-\sum_{s=1}^{t-1} z_s u)$.

By per-step analysis in online least squares
(See e.g. ~\cite{Orabona-Cesa-Bianchi-Gentile-2012}), we have that
\begin{align*}
  &\frac12(\inn{W_t}{z_t} + u)^2 (1 - z_t^T A_t^{-1} z_t)
  - \frac12(\inn{U}{z_t} + u)^2 \\
  &\quad \leq
  \frac 1 2 \| U - W_t \|_{A_{t-1}}^2 - \frac 1 2 \| U - W_{t+1} \|_{A_t}^2~.
\end{align*}

Denoting by $k_t=1-z_t^T A_t^{-1} z_t$ and summing over all rounds $t = 1,\ldots,T$,
\begin{align*}
   &\frac12 \sum_{t=1}^T I[g_t \neq 0]
   \left[ (\inn{W_t}{z_t} + u)^2 k_t - (\inn{U}{z_t} + u)^2 \right] \\
   &\quad \leq \frac 1 2 \| U \|_{A_0}^2 - \frac 1 2 \| U - W_{T+1} \|_{A_T}^2~.
\end{align*}
Now, notice that $k_t \geq 0$. Also $\frac12(\inn{W_t}{z_t} + u)^2 \geq u^2$, because
$\inn{W_t}{z_t} \geq 0$ and $u \geq 0$. So, we get
\[
\sum_{t=1}^T I[g_t \neq 0]
   \left[ \frac {u^2} 2 k_t - \frac12(\inn{U}{z_t} + u)^2 \right]
   \leq \frac a 2 \| U \|^2~.
\]
Thus,
\begin{align*}
& \frac12 \sum_{t=1}^T I[g_t \neq 0]
\left[ u^2 - ( (\inn{U}{z_t})^2 + 2 u \inn{U}{z_t} + u^2) \right] \\
&\quad \leq \frac a 2 \| U \|^2 + \frac {u^2} {2} \sum_{t=1}^T z_t^T A_t^{-1} z_t~.
\end{align*}
Therefore,
\begin{align*}
&\sum_{t=1}^T I[g_t \neq 0] \left[ - \frac12 (\inn{U}{z_t})^2 - u \inn{U}{z_t} \right]\\
&\quad \leq \frac a 2 \| U \|^2 + \frac {k} {2\gamma} \ln \frac{|A_T|}{|A_0|} \\
&\quad \leq \frac a 2 \| U \|^2 + \frac {k} {2\gamma} \cdot k d \ln\left(1 + \frac{2TX^2k}{a \gamma d}\right)~.
\end{align*}
where the first inequality is a well-known fact from linear algebra (see Lemma 11 of~\cite{Hazan-Agarwal-Kale-2007}),
the second inequality is from that the maximum eigenvalue of $A_T$ is at most
$a + \sum_t \| z_t \|^2 \leq a + \frac{2TX^2k}{\gamma}$ and that the dimension of
$A_T$ is $kd \times kd$.
The proof is concluded by recognizing $g_t = u z_t$ and algebra.
\end{proof}


\subsubsection{Derived Mistake Bound}
We get the following mistake bound on the proposed algorithm.
%
\begin{theorem}
Let $W^*$ any matrix in $\R^{k \times d}$.
For any $0 < \eta \leq \min(1, \tfrac{2}{\| W^* \| X + 1})$, the expected number of mistakes can be bounded as
\begin{align*}
\E\left[\sum_{t=1}^T I[\hat{y}_t \neq y_t]\right]
&\leq
%\E[\sum_{t=1}^T I(\hat{y}_t \neq y_t) l_\eta(W^*)]
\E[L_\eta^*(W^*)]+\frac{a\eta}{2-\eta} \| W^* \|^2 \\
&\quad + \frac{k}{\gamma} \frac{d}{\eta(2-\eta)} \ln\left(1 + \frac{TX^2 k}{a d \gamma}\right),
\end{align*}
where $L^*_\eta(W^*) := \sum_{t=1}^T \ell_\eta(\max_{i \neq y_t}\inn{W^*}{x_t \otimes (e_{y_t} - e_i)})$
is the $\eta$-loss of the linear predictor $W^*$.
%, and $d_m := \| W^* \|^2 X^2$.
%is the margin-based complexity of the hypothesis class.
\end{theorem}
%
\begin{proof}
Use Lemma~\ref{lem:vaw} with $U = \eta W^*$ and take expectations on both sides of Lemma~\ref{lem:vaw}
\begin{align*}
\E &\left[2 \sum_{t=1}^T \eta \inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t})}\right] \\
&\leq a  \eta^2 \| W^* \|^2 + \E \left[\sum_{t=1}^T \eta^2 (\inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t})})^2\right] \\
&\quad + \frac{k\, d} {\gamma} \ln\left(1 + \frac{T\, X^2\,k}{a\, \gamma\, d}\right),
\end{align*}
where we used \eqref{eq:expectation_g} and \eqref{eq:expectation_z2}.
Add the terms $\eta(2-\eta) \E\left[\sum_{t=1}^T I[\hat{y}_t \neq y_t]\right]$ to both terms and divide both term by $\eta(2-\eta)$, to have
\begin{align*}
\E&\left[\sum_{t=1}^T I[\hat{y}_t \neq y_t]\right] \\
&\leq \E\left[\sum_{t=1}^T I[\hat{y}_t \neq y_t] f(\inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t})})\right] \\
&\quad +\frac{a\eta}{2-\eta} \| W^* \|^2+\frac{k}{\gamma} \frac{d}{\eta(2-\eta)} \ln\left(1 + \frac{T\,X^2\, k}{a\, d\, \gamma}\right),
\end{align*}
where $f(z) = 1 - \frac{2}{2-\eta} z + \frac{\eta}{2-\eta} z^2$.
Taking a close look at the function $f$, we observe that the two roots of the quadratic function  are $1$ and $\frac{2-\eta}{\eta}$,
respectively. Setting $\eta\leq 1$, the function is negative between $1$ and $\frac{2-\eta}{\eta}$ and positive in $(-\infty, 1]$.
Thus, if we can set $\eta$ such that $\inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t}}) \leq \frac{2-\eta}{\eta}$, e.g. $0 < \eta \leq \frac{2}{\|W^*\| X + 1}$, we have that
\begin{align*}
&f(\inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t}})) \\
&\quad \leq  \left|f(\inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t}}))\right|_+ \\
&\quad =\ell_\eta(\inn{W^*}{x_t \otimes (e_{y_t} - e_{\hat{y}_t}}))~.
\end{align*}
%
% \[
% f(z)
% =
% \begin{cases}
% 1 - \frac{2}{2-\eta} z + \frac{\eta}{2-\eta}z^2 & z \leq 1 \\
% 0 & \text{otherwise}
% \end{cases}
% \]
% By the monotonicity of $\ell_\eta$ in the region $(-\infty, \frac{2-\eta}{\eta}]$,
% we get the above is at most $\ell_\eta(\max_{i \neq y_t}\inn{W^*}{x_t \otimes (e_{y_t} - e_i)})$.
Putting together the two constraints on $\eta$ we have the stated assumption.
\end{proof}

In order to minimize the bound, the parameter $a$ should be set close to zero so that the two trailing terms are roughly $O(\frac{kd\sqrt{d_m}}{\gamma})$.
Finally, note that when playing $\gamma$-greedy exploration, our algorithm is
at most $T\gamma$-worse than the performance of $\hat{y}_t$.
Combining the above observations, we arrive at the main result of this section.
\begin{theorem}
For any $W^* \in \R^{k \times d}$, let $0 < \eta \leq \min(1, \frac{2}{\|W^*\| X + 1})$. Then the proposed bandit
multiclass linear learning algorithm, with inputs
$\gamma = k\sqrt{\frac{\sqrt{dd_m}\ln(kT)}{T}} = O(\sqrt{\frac{1}{T}})$
and $\omega(T^\alpha) \leq a \leq o(\sqrt{T})$,
has the following upper bound on the expected number of mistakes:
\[
\E\left[ \sum_{t=1}^T I[\tilde{y}_t \neq y_t] \right]
\leq
\E\left[L^*_\eta(W^*)\right]
+
k\sqrt{\sqrt{dd_m}T \ln(kT)},
\]
where $L^*_\eta := \sum_{t=1}^T \ell_\eta(\max_{i \neq y_t}\inn{W^*}{x_t \otimes (e_{y_t} - e_i)})$
is the $\eta$-loss of the best linear predictor $W^*$, and
$d_m := D^2X^2$ is the margin-based complexity of the hypothesis class.
\end{theorem}

